CDRL: A Reinforcement Learning Framework Inspired by Cerebellar Circuits and Dendritic Computational Strategies

Reinforcement learning (RL) has achieved notable performance in high-dimensional sequential decision-making tasks, yet remains limited by low sample efficiency, sensitivity to noise, and weak generalization under partial observability. Most existing approaches address these issues primarily through optimization strategies, while the role of architectural priors in shaping representation learning and decision dynamics is less explored. Inspired by structural principles of the cerebellum, we propose a biologically grounded RL architecture that incorporate large expansion, sparse connectivity, sparse activation, and dendritic-level modulation. Experiments on noisy, high-dimensional RL benchmarks show that both the cerebellar architecture and dendritic modulation consistently improve sample efficiency, robustness, and generalization compared to conventional designs. Sensitivity analysis of architectural parameters suggests that cerebellum-inspired structures can offer optimized performance for RL with constrained model parameters. Overall, our work underscores the value of cerebellar structural priors as effective inductive biases for RL.

==> table_CIRL.tex <==
% % \usepackage[table]{xcolor}
% % \definecolor{m2blue}{HTML}{e1f5fe}

\begin{table*}[htdp]
\centering
\caption{Winrate comparison of CIRL model and baseline model under different observation and action noise.}
\label{tab:winrate_wide}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule
\makecell{Obs / \\ Act} & 0.00 & 0.05 & 0.10 & 0.15 & 0.20 & 0.30 \\
\midrule
0 & \makecell{0.92$\pm$0.04 \\ \cellcolor{m2blue}0.98$\pm$0.01} & \makecell{0.93$\pm$0.04 \\ \cellcolor{m2blue}0.97$\pm$0.01} & \makecell{0.90$\pm$0.04 \\ \cellcolor{m2blue}0.96$\pm$0.03} & \makecell{0.87$\pm$0.07 \\ \cellcolor{m2blue}0.97$\pm$0.01} & \makecell{0.84$\pm$0.06 \\ \cellcolor{m2blue}0.95$\pm$0.03} & \makecell{0.73$\pm$0.13 \\ \cellcolor{m2blue}0.92$\pm$0.05} \\
1 & \makecell{0.88$\pm$0.11 \\ \cellcolor{m2blue}0.90$\pm$0.10} & \makecell{0.83$\pm$0.16 \\ \cellcolor{m2blue}0.92$\pm$0.08} & \makecell{0.84$\pm$0.11 \\ \cellcolor{m2blue}0.90$\pm$0.09} & \makecell{0.80$\pm$0.14 \\ \cellcolor{m2blue}0.91$\pm$0.08} & \makecell{0.79$\pm$0.15 \\ \cellcolor{m2blue}0.88$\pm$0.09} & \makecell{0.62$\pm$0.09 \\ \cellcolor{m2blue}0.85$\pm$0.09} \\
2 & \makecell{0.58$\pm$0.31 \\ \cellcolor{m2blue}0.62$\pm$0.24} & \makecell{0.54$\pm$0.29 \\ \cellcolor{m2blue}0.64$\pm$0.23} & \makecell{0.54$\pm$0.31 \\ \cellcolor{m2blue}0.63$\pm$0.27} & \makecell{0.51$\pm$0.29 \\ \cellcolor{m2blue}0.62$\pm$0.27} & \makecell{0.52$\pm$0.23 \\ \cellcolor{m2blue}0.59$\pm$0.24} & \makecell{0.42$\pm$0.21 \\ \cellcolor{m2blue}0.60$\pm$0.21} \\
3 & \makecell{0.50$\pm$0.29 \\ \cellcolor{m2blue}0.48$\pm$0.23} & \makecell{0.48$\pm$0.30 \\ \cellcolor{m2blue}0.51$\pm$0.26} & \makecell{0.45$\pm$0.23 \\ \cellcolor{m2blue}0.46$\pm$0.26} & \makecell{0.46$\pm$0.25 \\ \cellcolor{m2blue}0.51$\pm$0.21} & \makecell{0.40$\pm$0.21 \\ \cellcolor{m2blue}0.46$\pm$0.24} & \makecell{0.40$\pm$0.18 \\ \cellcolor{m2blue}0.49$\pm$0.20} \\
5 & \makecell{0.30$\pm$0.09 \\ \cellcolor{m2blue}0.34$\pm$0.24} & \makecell{0.33$\pm$0.05 \\ \cellcolor{m2blue}0.31$\pm$0.23} & \makecell{0.30$\pm$0.07 \\ \cellcolor{m2blue}0.33$\pm$0.24} & \makecell{0.28$\pm$0.07 \\ \cellcolor{m2blue}0.30$\pm$0.18} & \makecell{0.32$\pm$0.04 \\ \cellcolor{m2blue}0.31$\pm$0.18} & \makecell{0.29$\pm$0.07 \\ \cellcolor{m2blue}0.32$\pm$0.15} \\
10 & \makecell{0.27$\pm$0.07 \\ \cellcolor{m2blue}0.29$\pm$0.05} & \makecell{0.31$\pm$0.06 \\ \cellcolor{m2blue}0.28$\pm$0.04} & \makecell{0.29$\pm$0.06 \\ \cellcolor{m2blue}0.31$\pm$0.07} & \makecell{0.26$\pm$0.06 \\ \cellcolor{m2blue}0.31$\pm$0.08} & \makecell{0.28$\pm$0.04 \\ \cellcolor{m2blue}0.28$\pm$0.06} & \makecell{0.27$\pm$0.01 \\ \cellcolor{m2blue}0.27$\pm$0.06} \\
\bottomrule
\end{tabular}}
\end{table*}


